Re-Nerfing: Improving Novel View Synthesis through Novel View Synthesis

Recent neural rendering and reconstruction techniques, such as NeRFs or Gaussian Splatting, have shown remarkable novel view synthesis capabilities but require hundreds of images of the scene from diverse viewpoints to render high-quality novel views. With fewer images available, these methods start to fail since they can no longer correctly triangulate the underlying 3D geometry and converge to a non-optimal solution. These failures can manifest as floaters or blurry renderings in sparsely observed areas of the scene. In this paper, we propose Re-Nerfing, a simple and general add-on approach that leverages novel view synthesis itself to tackle this problem. Using an already trained NVS method, we render novel views between existing ones and augment the training data to optimize a second model. This introduces additional multi-view constraints and allows the second model to converge to a better solution. With Re-Nerfing we achieve significant improvements upon multiple pipelines based on NeRF and Gaussian-Splatting in sparse view settings of the mip-NeRF 360 and LLFF datasets. Notably, Re-Nerfing does not require prior knowledge or extra supervision signals, making it a flexible and practical add-on.

==> tables/even_more_rounds.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3.1pt}
\begin{center}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
& \multicolumn{3}{c|}{3DGS~\cite{kerbl2023gaussiansplat}} & \multicolumn{3}{c|c }{PyNeRF~\cite{turki2024pynerf}} &
\multicolumn{3}{c}{Instant-NGP~\cite{muller2022instant}}\\
%Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
Method & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS  &PSNR & SSIM & LPIPS \\
\midrule

baseline & 19.31 & 0.609 & 0.296 & 17.57 & 0.643 & 0.325 & 17.68 & 0.555 & 0.460 \\
%baseline, 2x iterations & 19.68 & 0.633 & 0.274 & 17.93	& 0.653 & 0.331 \\
+ [ours]: 1 & 21.08 & 0.686 & 0.241 & 18.09 & 0.676 & 0.299 & 18.40 & 0.580 & 0.416 \\
+ [ours]: 2 & 21.89 & 0.720 & 0.214 & 18.36 & 0.693 & 0.285 & 18.41 & 0.590 & 0.402 \\
+ [ours]: 3 & 22.47 & 0.748 & 0.191 & 18.41 & 0.699 & 0.281 & \uline{18.86} & \textbf{0.603} & \textbf{0.389} \\
+ [ours]: 4 & \uline{22.63} & \uline{0.756} & \uline{0.184} & \uline{18.47} & \uline{0.704} & \uline{0.275} & \textbf{18.88} & \uline{0.600} & \uline{0.394} \\
+ [ours]: 5 & \textbf{22.76} & \textbf{0.761} & \textbf{0.178} & \textbf{18.64} & \textbf{0.708} & \textbf{0.272} & 18.82 & 0.598 & 0.397 \\

\bottomrule
\end{tabular}
\vspace{-0.7em}
\caption{Rendering performance on the mip-NeRF 360~\cite{barron2022mip360} \textit{counter} scene in the 30-view setting. \pname\ is applied iteratively (5x).
%and the effect of training the baseline for double the amount of iterations is also shown (2x). All other models in this work were trained for 30k iterations.
}
\label{tab:more_rounds}
\vspace{-1.5em}
\end{center}
\end{table*}

==> tables/gsplat.tex <==
\begin{wraptable}{l}{0.6\textwidth}
%\begin{table*}
\setlength{\tabcolsep}{5pt}
%\begin{center}
\begin{tabular}{l|ccc}
\toprule
& \multicolumn{3}{c}{sparser views} \\
%Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
Method & PSNR & SSIM & LPIPS \\
\midrule

3DGS~\cite{kerbl2023gaussiansplat} & 20.49 & 0.600 & 0.259 \\
+ \pname\ [ours] & \textbf{21.30} & \textbf{0.627} & \textbf{0.235} \\

\bottomrule
\end{tabular}
\vspace{0.2cm}
\caption{Rendering performance on the mip-NeRF 360~\cite{barron2022mip360} dataset in sparser settings averaged over all scenes. The proposed \pname\ is applied on 3D Gaussian Splatting~\cite{kerbl2023gaussiansplat}, using the baseline to augment the views. No uncertainty estimates were used, unavailable due to the method's explicit representation.}
%, with every 8th image used as test-view. To showcase the performance of our method on sparser views, we also report results for half, a quarter and an eights of the original views. The 1/8 views setting is only applied to the bonsai and room scene as for all others NeRF reconstruction failed. For DS-NeRF~\cite{deng2022dsnerf} we use the provided depth from colmap for the full scenes but find that it fails on some of the sparser-view scenes so do not report metrics there.
\label{tab:gsplat}
%\vspace{-0.7cm}
%\end{center}
%\end{table*}
\end{wraptable}

==> tables/gsplat_all_views.tex <==
%\begin{wraptable}{l}{0.6\textwidth}
\begin{table*}
\setlength{\tabcolsep}{5pt}
\begin{center}
\begin{tabular}{l|ccc}
\toprule
& \multicolumn{3}{c}{denser views} \\
%Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
Method & PSNR & SSIM & LPIPS \\
\midrule

3DGS~\cite{kerbl2023gaussiansplat} & 27.83 & 0.855 & \textbf{0.109} \\
+ \pname\ [ours] & \textbf{28.03} & \textbf{0.859} & 0.111 \\

\bottomrule
\end{tabular}
\vspace{0.2cm}
\caption{Rendering performance on the mip-NeRF 360~\cite{barron2022mip360} dataset in denser settings averaged over all scenes. The proposed \pname\ is applied on 3D Gaussian Splatting~\cite{kerbl2023gaussiansplat}, using the baseline to augment the views. No uncertainty estimates were used, unavailable due to the method's explicit representation.}
%, with every 8th image used as test-view. To showcase the performance of our method on sparser views, we also report results for half, a quarter and an eights of the original views. The 1/8 views setting is only applied to the bonsai and room scene as for all others NeRF reconstruction failed. For DS-NeRF~\cite{deng2022dsnerf} we use the provided depth from colmap for the full scenes but find that it fails on some of the sparser-view scenes so do not report metrics there.
\label{tab:gsplat_all_views}
%\vspace{-0.7cm}
\end{center}
\end{table*}
%\end{wraptable}

==> tables/more_views.tex <==
%\begin{wraptable}{l}{0.6\textwidth}
\begin{table*}
\setlength{\tabcolsep}{5pt}
\begin{center}
\begin{tabular}{l|ccc}
\toprule
& \multicolumn{3}{c}{sparser views} \\
%Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
Method & PSNR & SSIM & LPIPS \\
\midrule

PyNeRF~\cite{turki2024pynerf} & 22.42 & 0.632 & 0.218 \\
%Zip-NeRF + DS-NeRF~\cite{deng2022dsnerf} & 30.16 & 0.903 & 0.058 & - & - & - & - & - & - & - & - & - \\
%\midrule
adding 4 randomly interpolated synthetic views (1.08x) & 22.58 & 0.653 & 0.205 \\
adding 4 test synthetic views (1.08x) & \textbf{22.64} & \textbf{0.663} & \textbf{0.196} \\
%adding 50 syn.~views (2x) & 23.35 & 0.669 & 0.190 \\
%adding 100 syn.~views (3x) & 23.61 & 0.670 & 0.189\\

\bottomrule
\end{tabular}
\vspace{0.2cm}
\caption{View optimization strategies on the sparser setting of the \textit{stump} scene of the mip-NeRF 360~\cite{barron2022mip360} dataset (50 views). All models are based on PyNeRF~\cite{turki2024pynerf}.}
%Rendering performance on the mip-NeRF 360~\cite{barron2022mip360} dataset in denser settings averaged over all scenes. The proposed \pname\ is applied on 3D Gaussian Splatting~\cite{kerbl2023gaussiansplat}, using the baseline to augment the views. No uncertainty estimates were used, unavailable due to the method's explicit representation.}
%, with every 8th image used as test-view. To showcase the performance of our method on sparser views, we also report results for half, a quarter and an eights of the original views. The 1/8 views setting is only applied to the bonsai and room scene as for all others NeRF reconstruction failed. For DS-NeRF~\cite{deng2022dsnerf} we use the provided depth from colmap for the full scenes but find that it fails on some of the sparser-view scenes so do not report metrics there.
\label{tab:more_views}
\vspace{-1.0cm}
\end{center}
\end{table*}
%\end{wraptable}
